Robust Streaming Erasure Codes based on Deterministic Channel Approximations

We study near optimal error correction codes for real-time communication. In our setup the encoder must operate on an incoming source stream in a sequential manner, and the decoder must reconstruct each source packet within a fixed playback deadline of $T$ packets. The underlying channel is a packet erasure channel that can introduce both burst and isolated losses. We first consider a class of channels that in any window of length ${T+1}$ introduce either a single erasure burst of a given maximum length $B,$ or a certain maximum number $N$ of isolated erasures. We demonstrate that for a fixed rate and delay, there exists a tradeoff between the achievable values of $B$ and $N,$ and propose a family of codes that is near optimal with respect to this tradeoff. We also consider another class of channels that introduce both a burst {\em and} an isolated loss in each window of interest and develop the associated streaming codes. All our constructions are based on a layered design and provide significant improvements over baseline codes in simulations over the Gilbert-Elliott channel.

==> partial-recoveryA1.tex <==
\node[triple2, minimum width=1.6cm] (start) {
	$u$ Symbols
    \nodepart{second}
      $v$ Symbols
    \nodepart{third}
     \tikz{\node[double2] {$u$ \nodepart{second}Symbols};}
		\nodepart{fourth}
		\tikz{\node[block2] {$s$ Symbols};}
      %$B$ Symbols
  };
	
  \node[triple,  right = of start,fill=light-gray,minimum width=1.6cm] (p1) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{-1})$};}
  };
  
  %\node [block, right of=p1,minimum width=1.65cm, minimum height=3.28cm,node distance=1.94cm, fill=light-gray] (p2) {$\cdots$};
	\node[triple, font=\color{light-gray}, right = of p1,fill=light-gray,minimum width=1.6cm] (p2) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{-1})$};}
  };
	
  \node[triple, right = of p2,fill=light-gray,minimum width=1.6cm] (p3) {$\bu[B-1]$
    \nodepart{second}
      $\bv[B-1]$
    \nodepart{third}
      \tikz{\node[double2] {$\bu[B-\Delta-1]$ \nodepart{second}$+\bp_1(\bv^{B-2})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{B-2})$};}
  };
  
  \node[triple,  right = of p3,minimum width=1.6cm] (p4) {$\bu[B]$
    \nodepart{second}
      $\bv[B]$
    \nodepart{third}
      \tikz{\node[double2,pattern=north east lines wide, pattern color=gray] {$\bu[B-\Delta]$ \nodepart{second}$+\bp_1(\bv^{B-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2,pattern=north east lines wide, pattern color=gray] {$\bp_2(\bv^{B-1})$};}
  };
  
  %\node [block, right of=p4,minimum width=1.65cm, minimum height=3.28cm,node distance=1.96cm] (p5) {$\cdots$};
	\node[triple, font=\color{white}, right = of p4,minimum width=1.6cm] (p5) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2,pattern=north east lines wide, pattern color=gray] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2,pattern=north east lines wide, pattern color=gray] {$\bp_2(\bv^{-1})$};}
  };
	
  \node[triple,  right = of p5,minimum width=1.6cm] (p6) {$\bu[t-1]$
    \nodepart{second}
      $\bv[t-1]$
    \nodepart{third}
      \tikz{\node[double2,pattern=north east lines wide, pattern color=gray] {$\bu[t-\Delta-1]$ \nodepart{second}$+\bp_1(\bv^{t-2})$};}
			\nodepart{fourth}
			\tikz{\node[block2,pattern=north east lines wide, pattern color=gray] {$\bp_2(\bv^{t-2})$};}
  };
  
  \node[triple, right = of p6,fill=light-gray,minimum width=1.6cm] (p7) {$\bu[t]$
    \nodepart{second}
      $\bv[t]$
    \nodepart{third}
      \tikz{\node[double2] {$\bu[t-\Delta]+$ \nodepart{second}$\bp_1(\bv^{t-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{t-1})$};}
  };
  
  %\node [block, right of=p7,minimum width=1.65cm, minimum height=3.28cm,node distance=1.96cm] (p8) {$\cdots$};
	\node[triple, font=\color{white}, right = of p7,minimum width=1.6cm] (p8) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2,pattern=north east lines wide, pattern color=gray] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2,pattern=north east lines wide, pattern color=gray] {$\bp_2(\bv^{-1})$};}
  };
  
  \node[triple, right = of p8,minimum width=1.6cm] (p9) {$\bu[\Delta-1]$
    \nodepart{second}
      $\bv[\Delta-1]$
    \nodepart{third}
      \tikz{\node[double2,pattern=north east lines wide, pattern color=gray] {$\bu[-1]+$ \nodepart{second}$\bp_1(\bv^{\Delta-2})$};}
			\nodepart{fourth}
			\tikz{\node[block2,pattern=north east lines wide, pattern color=gray] {$\bp_2(\bv^{\Delta-2})$};}
  };
  
  \node[triple, right = of p9,minimum width=1.6cm] (p10) {$\bu[\Delta]$
    \nodepart{second}
      $\bv[\Delta]$
    \nodepart{third}
      \tikz{\node[double2,pattern=soft horizontal lines,pattern color=gray] {$\bu[0]+$ \nodepart{second}$\bp_1(\bv^{\Delta-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{\Delta-1})$};}
  };
  
  %\node [block, right of=p10,minimum width=1.65cm, minimum height=3.28cm,node distance=1.96cm] (p11) {$\cdots};
	\node[triple, font=\color{white}, right = of p10,minimum width=1.6cm] (p11) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2,pattern=soft horizontal lines,pattern color=gray] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{-1})$};}
  };
	
  \node[triple, right = of p11,minimum width=1.6cm] (p12) {$\bu[T]$
    \nodepart{second}
      $\bv[T]$
    \nodepart{third}
      \tikz{\node[double2,pattern=soft horizontal lines,pattern color=gray] {$\bu[T-\Delta]+$ \nodepart{second}$\bp_1(\bv^{T-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{T-1})$};}
  };
  
  %\node [block, right of=p12,minimum width=1.65cm, minimum height=3.28cm,node distance=1.96cm] (p13) {$\cdots$};
	\node[triple, font=\color{white}, right = of p12,minimum width=1.6cm] (p13) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2,pattern=soft horizontal lines,pattern color=gray] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{-1})$};}
  };
  
  \node[triple, right = of p13,minimum width=1.6cm] (p14) {$\bu[\Delta+B-1]$
    \nodepart{second}
      $\bv[\Delta+B-1]$
    \nodepart{third}
      \tikz{\node[double2,pattern=soft horizontal lines,pattern color=gray] {$\bu[B-1]+$ \nodepart{second}$\bp_1(\bv^{\Delta+B-2})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{\Delta+B-2})$};}
  };
  
  \bracedn{p1}{p3}{-2mm}{\footnotesize{Erasure Burst}};
  \bracedn{p4}{p9}{-2mm}{\footnotesize{Recover $\bv[0],\cdots ,\bv[B-1],\bv[t]$}};
  \bracedn{p10}{p10}{-2mm}{\footnotesize{$\bu[0]$}};
	\bracedn{p14}{p14}{-2mm}{\footnotesize{$\bu[B-1]$}};

==> partial-recoveryA2.tex <==
\node[triple2, minimum width=1.6cm] (start) {
	$u$ Symbols
    \nodepart{second}
      $v$ Symbols
    \nodepart{third}
     \tikz{\node[double2] {$u$ \nodepart{second}Symbols};}
		\nodepart{fourth}
		\tikz{\node[block2] {$s$ Symbols};}
      %$B$ Symbols
  };
	
  \node[triple,  right = of start,fill=light-gray,minimum width=1.6cm] (p1) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{-1})$};}
  };
	
	\node[triple, font=\color{light-gray}, right = of p1,fill=light-gray,minimum width=1.6cm] (p2) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{-1})$};}
  };
  
  \node[triple, right = of p2,fill=light-gray,minimum width=1.6cm] (p3) {$\bu[B-1]$
    \nodepart{second}
      $\bv[B-1]$
    \nodepart{third}
      \tikz{\node[double2] {$\bu[B-\Delta+1]$ \nodepart{second}$+\bp_1(\bv^{B-2})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{B-2})$};}
  };
  
  \node[triple, font=\color{white}, right = of p3,minimum width=1.6cm] (p4) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2,pattern=north east lines wide, pattern color=gray] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2,pattern=north east lines wide, pattern color=gray] {$\bp_2(\bv^{-1})$};}
  };
  
  %
  \node[triple,  right = of p4,minimum width=1.6cm] (p5) {$\bu[\tau]$
    \nodepart{second}
      $\bv[\tau]$
    \nodepart{third}
      \tikz{\node[double2,pattern=north east lines wide, pattern color=gray] {$\bu[\tau-\Delta]$ \nodepart{second}$+\bp_1(\bv^{\tau-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2,pattern=north east lines wide, pattern color=gray] {$\bp_2(\bv^{\tau-1})$};}
  };
  
  \node[triple, font=\color{white}, right = of p5,minimum width=1.6cm] (p6) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{-1})$};}
  };

\iffalse  
  \node[triple, right = of p6,minimum width=1.6cm] (p7) {$\bu[\Delta-1]$
    \nodepart{second}
      $\bv[\Delta-1]$
    \nodepart{third}
      \tikz{\node[double2] {$\bu[-1]+$ \nodepart{second}$\bp_1(\bv^{\Delta-2})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{\Delta-2})$};}
  };
	\fi
  
  \node[triple, right = of p6,minimum width=1.6cm] (p8) {$\bu[\Delta]$
    \nodepart{second}
      $\bv[\Delta]$
    \nodepart{third}
      \tikz{\node[double2,pattern=soft horizontal lines,pattern color=gray] {$\bu[0]+$ \nodepart{second}$\bp_1(\bv^{\Delta-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{\Delta-1})$};}
  };
  
  \node[triple, font=\color{white}, right = of p8,minimum width=1.6cm] (p9) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2,pattern=soft horizontal lines,pattern color=gray] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{-1})$};}
  };
	
	\node[triple,  right = of p9,minimum width=1.6cm] (p10) {$\bu[t-1]$
    \nodepart{second}
      $\bv[t-1]$
    \nodepart{third}
      \tikz{\node[double2,pattern=soft horizontal lines, pattern color=gray] {$\bu[t-\Delta-1]$ \nodepart{second}$+\bp_1(\bv^{t-2})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{t-2})$};}
  };
  
  \node[triple, right = of p10,fill=light-gray,minimum width=1.6cm] (p11) {$\bu[t]$
    \nodepart{second}
      $\bv[t]$
    \nodepart{third}
      \tikz{\node[double2] {$\bu[t-\Delta]+$ \nodepart{second}$\bp_1(\bv^{t-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{t-1})$};}
  };
	
	\node[triple, right = of p11,minimum width=1.6cm] (p12) {$\bu[t+1]$
    \nodepart{second}
      $\bv[t+1]$
    \nodepart{third}
      \tikz{\node[double2,pattern=soft horizontal lines,pattern color=gray] {$\bu[t-\Delta+1]$ \nodepart{second}$+\bp_1(\bv^{t})$};}
			\nodepart{fourth}
			\tikz{\node[block2,pattern=north east lines wide, pattern color=gray] {$\bp_2(\bv^{t})$};}
  };
	
	\node[triple, font=\color{white}, right = of p12,minimum width=1.6cm] (p13) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2,pattern=soft horizontal lines,pattern color=gray] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2,pattern=north east lines wide, pattern color=gray] {$\bp_2(\bv^{-1})$};}
  };
	
  \node[triple, right = of p13,minimum width=1.6cm] (p14) {$\bu[t+T-\Delta+1]$
    \nodepart{second}
      $\bv[t+T-\Delta+1]$
    \nodepart{third}
      \tikz{\node[double2,pattern=soft horizontal lines,pattern color=gray] {$\bu[t+T-2\Delta+1]$ \nodepart{second}$+\bp_1(\bv^{t+T-\Delta})$};}
			\nodepart{fourth}
			\tikz{\node[block2,pattern=north east lines wide, pattern color=gray] {$\bp_2(\bv^{t+T-\Delta})$};}
  };
  
  %\node [block, right of=p12,minimum width=1.65cm, minimum height=3.28cm,node distance=1.96cm] (p13) {$\cdots$};
	\node[triple, font=\color{white}, right = of p14,minimum width=1.6cm] (p15) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2,pattern=soft horizontal lines,pattern color=gray] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{-1})$};}
  };
  
  \node[triple, right = of p15,minimum width=1.6cm] (p16) {$\bu[\Delta+B-1]$
    \nodepart{second}
      $\bv[\Delta+B-1]$
    \nodepart{third}
      \tikz{\node[double2,pattern=soft horizontal lines,pattern color=gray] {$\bu[B-1]+$ \nodepart{second}$\bp_1(\bv^{\Delta+B-2})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{\Delta+B-2})$};}
  };
  
  \bracedn{p1}{p3}{-3mm}{\footnotesize{Erasure Burst}};
  \bracedn{p4}{p5}{-3mm}{\footnotesize{Recover $\bv[0],\cdots ,\bv[B-1]$}};
	\bracedn{p12}{p14}{-3mm}{\footnotesize{Recover $\bv[t]$}};
  \bracedn{p8}{p8}{-3mm}{\footnotesize{$\bu[0]$}};
	\bracedn{p10}{p10}{-3mm}{\footnotesize{$\bu[t-\Delta-1]$}};
	\bracedn{p12}{p12}{-8mm}{\footnotesize{$\bu[t-\Delta+1]$}};
	\bracedn{p16}{p16}{-8mm}{\footnotesize{$\bu[B-1]$}};

==> partial-recoveryB1.tex <==
\node[triple2, minimum width=1.6cm] (start) {
	$u$ Symbols
    \nodepart{second}
      $v$ Symbols
    \nodepart{third}
     \tikz{\node[double2] {$u$ \nodepart{second}Symbols};}
		\nodepart{fourth}
		\tikz{\node[block2] {$s$ Symbols};}
      %$B$ Symbols
  };
	
	\node[triple, right = of start,fill=light-gray,minimum width=1.6cm] (p1) {$\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2] {$\bu[-\Delta]+$ \nodepart{second}$\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{-1})$};}
  };
  
  \node[triple, font=\color{white}, right = of p1,minimum width=1.6cm] (p2) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2,pattern=north east lines wide, pattern color=gray] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2,pattern=north east lines wide, pattern color=gray] {$\bp_2(\bv^{-1})$};}
  };
	
  \node[triple,  right = of p2,fill=light-gray,minimum width=1.6cm] (p3) {
  $\bu[t]$
    \nodepart{second}
      $\bv[t]$
    \nodepart{third}
      \tikz{\node[double2] {$\bu[t-\Delta]$ \nodepart{second}$+\bp_1(\bv^{t-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{t-1})$};}
  };
	
	\node[triple, font=\color{light-gray}, right = of p3, fill=light-gray,minimum width=1.6cm] (p4) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{-1})$};}
  };
  
  \node[triple, right = of p4,fill=light-gray,minimum width=1.6cm] (p5) {$\bu[t+B-1]$
    \nodepart{second}
      $\bv[t+B-1]$
    \nodepart{third}
      \tikz{\node[double2] {$\bu[t+B-\Delta-1]$ \nodepart{second}$+\bp_1(\bv^{t+B-2})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{t+B-2})$};}
  };
  
  \node[triple,  right = of p5,minimum width=1.6cm] (p6) {$\bu[t+B]$
    \nodepart{second}
      $\bv[t+B]$
    \nodepart{third}
      \tikz{\node[double2,pattern=north east lines wide, pattern color=gray] {$\bu[t+B-\Delta]$ \nodepart{second}$+\bp_1(\bv^{t+B-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2,pattern=north east lines wide, pattern color=gray] {$\bp_2(\bv^{t+B-1})$};}
  };
  
  \node[triple, font=\color{white}, right = of p6,minimum width=1.6cm] (p7) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2,pattern=north east lines wide, pattern color=gray] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2,pattern=north east lines wide, pattern color=gray] {$\bp_2(\bv^{-1})$};}
  };
  
  \node[triple, right = of p7,minimum width=1.6cm] (p9) {$\bu[\Delta-1]$
    \nodepart{second}
      $\bv[\Delta-1]$
    \nodepart{third}
      \tikz{\node[double2,pattern=north east lines wide, pattern color=gray] {$\bu[-1]+$ \nodepart{second}$\bp_1(\bv^{\Delta-2})$};}
			\nodepart{fourth}
			\tikz{\node[block2,pattern=north east lines wide, pattern color=gray] {$\bp_2(\bv^{\Delta-2})$};}
  };
  
  \node[triple, right = of p9,minimum width=1.6cm] (p10) {$\bu[\Delta]$
    \nodepart{second}
      $\bv[\Delta]$
    \nodepart{third}
      \tikz{\node[double2,pattern=soft horizontal lines,pattern color=gray] {$\bu[0]+$ \nodepart{second}$\bp_1(\bv^{\Delta-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{\Delta-1})$};}
  };
  
  \node[triple, font=\color{white}, right = of p10,minimum width=1.6cm] (p11) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{-1})$};}
  };
	
  \node[triple, right = of p11,minimum width=1.6cm] (p12) {$\bu[t+\Delta]$
    \nodepart{second}
      $\bv[t+\Delta]$
    \nodepart{third}
      \tikz{\node[double2,pattern=soft horizontal lines,pattern color=gray] {$\bu[t]+$ \nodepart{second}$\bp_1(\bv^{t+\Delta-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{t+\Delta-1})$};}
  };
  
  \node[triple, font=\color{white}, right = of p12,minimum width=1.6cm] (p13) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2,pattern=soft horizontal lines,pattern color=gray] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{-1})$};}
  };
  
  \node[triple, right = of p13,minimum width=1.6cm] (p14) {$\bu[t+\Delta+B-1]$
    \nodepart{second}
      $\bv[t+\Delta+B-1]$
    \nodepart{third}
      \tikz{\node[double2,pattern=soft horizontal lines,pattern color=gray] {$\bu[t+B-1]+$ \nodepart{second}$\bp_1(\bv^{t+\Delta+B-2})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{t+\Delta+B-2})$};}
  };
  
	\bracedn{p1}{p1}{-2mm}{\footnotesize{Isolated Erasure}};
  \bracedn{p3}{p5}{-2mm}{\footnotesize{Erasure Burst}};
  \bracedn{p2}{p9}{-8mm}{\footnotesize{Recover $\bv[0],\bv[t],\cdots,\bv[t+B-1]$}};
  \bracedn{p10}{p10}{-2mm}{\footnotesize{$\bu[0]$}};
	\bracedn{p12}{p12}{-2mm}{\footnotesize{$\bu[t]$}};
	\bracedn{p14}{p14}{-2mm}{\footnotesize{$\bu[t+B-1]$}};

==> partial-recoveryB2.tex <==
\node[triple2, minimum width=1.6cm] (start) {
	$u$ Symbols
    \nodepart{second}
      $v$ Symbols
    \nodepart{third}
     \tikz{\node[double2] {$u$ \nodepart{second}Symbols};}
		\nodepart{fourth}
		\tikz{\node[block2] {$s$ Symbols};}
      %$B$ Symbols
  };
	
	\node[triple, right = of start,fill=light-gray,minimum width=1.6cm] (p1) {$\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2] {$\bu[-\Delta]+$ \nodepart{second}$\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{-1})$};}
  };
  
  \node[triple, font=\color{white}, right = of p1,minimum width=1.6cm] (p2) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2,pattern=north east lines wide, pattern color=gray] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2,pattern=north east lines wide, pattern color=gray] {$\bp_2(\bv^{-1})$};}
  };
  
  \node[triple,  right = of p2,minimum width=1.6cm] (p3) {$\bu[\tau]$
    \nodepart{second}
      $\bv[\tau]$
    \nodepart{third}
      \tikz{\node[double2,pattern=north east lines wide, pattern color=gray] {$\bu[\tau-\Delta]$ \nodepart{second}$+\bp_1(\bv^{\tau-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2,pattern=north east lines wide, pattern color=gray] {$\bp_2(\bv^{\tau-1})$};}
  };

	\node[triple, font=\color{white}, right = of p3,minimum width=1.6cm] (p4) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{-1})$};}
  };
	
  \node[triple,  right = of p4,fill=light-gray,minimum width=1.6cm] (p5) {
  $\bu[t]$
    \nodepart{second}
      $\bv[t]$
    \nodepart{third}
      \tikz{\node[double2] {$\bu[t-\Delta]$ \nodepart{second}$+\bp_1(\bv^{t-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{t-1})$};}
  };
  
  \node[triple, font=\color{light-gray}, right = of p5, fill=light-gray,minimum width=1.6cm] (p6) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{-1})$};}
  };
  
  \node[triple, right = of p6,fill=light-gray,minimum width=1.6cm] (p7) {$\bu[t+B-1]$
    \nodepart{second}
      $\bv[t+B-1]$
    \nodepart{third}
      \tikz{\node[double2] {$\bu[t+B-\Delta+1]$ \nodepart{second}$+\bp_1(\bv^{t+B-2})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{t+B-2})$};}
  };
  
  \node[triple, font=\color{white}, right = of p7,minimum width=1.6cm] (p8) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2,pattern=north east lines wide, pattern color=gray] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2,pattern=north east lines wide, pattern color=gray] {$\bp_2(\bv^{-1})$};}
  };
  
  \node[triple, right = of p8,minimum width=1.6cm] (p9) {$\bu[\Delta]$
    \nodepart{second}
      $\bv[\Delta]$
    \nodepart{third}
      \tikz{\node[double2, fill = light-gray] {$\bu[0]+$ \nodepart{second}$\bp_1(\bv^{\Delta-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{\Delta-1})$};}
  };
  
  \node[triple, font=\color{white}, right = of p9,minimum width=1.6cm] (p10) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2,pattern=north east lines wide, pattern color=gray] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2,pattern=north east lines wide, pattern color=gray] {$\bp_2(\bv^{-1})$};}
  };
	
	\node[triple, right = of p10,minimum width=1.6cm] (p11) {$\bu[t+\Delta-1]$
    \nodepart{second}
      $\bv[t+\Delta-1]$
    \nodepart{third}
      \tikz{\node[double2,pattern=north east lines wide, pattern color=gray] {$\bu[t-1]+$ \nodepart{second}$\bp_1(\bv^{t+\Delta-2})$};}
			\nodepart{fourth}
			\tikz{\node[block2,pattern=north east lines wide, pattern color=gray] {$\bp_2(\bv^{t+\Delta-2})$};}
  };
	
  \node[triple, right = of p11,minimum width=1.6cm] (p12) {$\bu[t+\Delta]$
    \nodepart{second}
      $\bv[t+\Delta]$
    \nodepart{third}
      \tikz{\node[double2,pattern=soft horizontal lines,pattern color=gray] {$\bu[t]+$ \nodepart{second}$\bp_1(\bv^{t+\Delta-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{t+\Delta-1})$};}
  };
  
  \node[triple, font=\color{white}, right = of p12,minimum width=1.6cm] (p13) {
  $\bu[0]$
    \nodepart{second}
      $\bv[0]$
    \nodepart{third}
      \tikz{\node[double2,pattern=soft horizontal lines,pattern color=gray] {$\bu[-\Delta]$ \nodepart{second}$+\bp_1(\bv^{-1})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{-1})$};}
  };
  
  \node[triple, right = of p13,minimum width=1.6cm] (p14) {$\bu[t+\Delta+B-1]$
    \nodepart{second}
      $\bv[t+\Delta+B-1]$
    \nodepart{third}
      \tikz{\node[double2,pattern=soft horizontal lines,pattern color=gray] {$\bu[t+B-1]+$ \nodepart{second}$\bp_1(\bv^{t+\Delta+B-2})$};}
			\nodepart{fourth}
			\tikz{\node[block2] {$\bp_2(\bv^{t+\Delta+B-2})$};}
  };
  %\node[block2, right = of p14] (p15) {$a$};
  
  %\braceright{p14}{p14}{$\cC_{12}$};
  
	\bracedn{p1}{p1}{-2mm}{\footnotesize{Isolated Erasure}};
	\bracedn{p2}{p3}{-2mm}{\footnotesize{Recover $\bv[0]$}};
  \bracedn{p5}{p7}{-2mm}{\footnotesize{Erasure Burst}};
  \bracedn{p8}{p11}{-2mm}{\footnotesize{Recover $\bv[t],\cdots,\bv[t+B-1]$}};
  %\bracedn{p10}{p10}{-2mm}{\footnotesize{$\bu[0]$}};
	\bracedn{p12}{p12}{-2mm}{\footnotesize{$\bu[t]$}};
	\bracedn{p14}{p14}{-2mm}{\footnotesize{$\bu[t+B-1]$}};
